Balanced Butterfly Counting in Bipartite-Network

Bipartite graphs offer a powerful framework for modeling complex relationships between two distinct types of vertices, incorporating probabilistic, temporal, and rating-based information. While the research community has extensively explored various types of bipartite relationships, there has been a notable gap in studying Signed Bipartite Graphs, which capture liking / disliking interactions in real-world networks such as customer-rating-product and senator-vote-bill. Balance butterflies, representing 2 x 2 bicliques, provide crucial insights into antagonistic groups, balance theory, and fraud detection by leveraging the signed information. However, such applications require counting balance butterflies which remains unexplored. In this paper, we propose a new problem: counting balance butterflies in a signed bipartite graph. To address this problem, we adopt state-of-the-art algorithms for butterfly counting, establishing a smart baseline that reduces the time complexity for solving our specific problem. We further introduce a novel bucket approach specifically designed to count balanced butterflies efficiently. We propose a parallelized version of the bucketing approach to enhance performance. Extensive experimental studies on nine real-world datasets demonstrate that our proposed bucket-based algorithm is up to 120x faster over the baseline, and the parallel implementation of the bucket-based algorithm is up to 45x faster over the single core execution. Moreover, a real-world case study showcases the practical application and relevance of counting balanced butterflies.

==> approximation.tex <==
\section{Approximation by Sparsification}
We design an algorithm for estimating the global number of signed butterflies using one-shot sparsification - where we sparsify the input graph into a small graph through a global sampling step. The number of signed butterflies in the sampled graph is used to estimate the number of signed butterflies in the original network. The sparsification method samples each edge in the network independently with a fixed probability $\rho$ and constructs a network with the sampled edges $E'$ only. Next, we count the signed butterflies in $G' = (V, E')$ and use this count to estimate the number of signed butterflies in the original network $G = (V, E)$. The pseudocode of {\tt SBESPAR} is described in Algorithm~\ref{sbespar}.

\begin{algorithm}[t]
\small
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{$G$$(U,V,E)$, Input signed bipartite graph, probability $\rho$, $0 < \rho < 1$}
	\Output{$\hat{\hourglass}_G$,  estimated number of balanced butterflies in $G$.}
	\SetKwFunction{FMain}{Balance\_Butterfly}
    \SetKwProg{Fn}{Function}{}{}
    \Fn{\FMain{$G$}}{
        Calculate $p(u)$ for each $u \in \{U \cup V\}$\\
        Rearrange $\Gamma(u)$ for each $u \in \{U \cup V\}$ in ascending order\\
       $\hourglass_G \gets 0$\\
       \ForEach{$u \in \{U \cup V\}$}{
       Initialise $H(w)$ for storing wedges corresponding to $v$\\
        \ForEach{$v \in \Gamma(u)$ $|$ $p(v)<p(u)$}{
        \ForEach{$w \in \Gamma(v)$ $|$ $p(w) < p(u)$}{
        \If{equal edges}{
        $B_1.add(H(w).add(v))$
        }
        \Else{
        $B_2.add(H(w).add(v))$
        }
        }
        }
        \tcc{For both the Buckets $B_1$ and $B_2$}
        \ForEach{$w$ $|$ $H(w)>1$}{
        \If{$|H(w)| >1$}{
        $\hourglass_G \gets \hourglass_G$ $+$ $\Mycomb[|H(w)|]{2}$
        }
        }
        }
  }
\caption{Bucket Approach}
\label{Algorithm:Bucket}
   \end{algorithm}

==> case-studies.tex <==
\section{Case Studies}
In network analysis, relationships between individuals or entities are typically represented as edges in a graph. A pattern or relation between nodes can be used as a tool to derive metric or to analyse data. The case study section utilises counting balanced butterflies algorithm in a bipartite graph to explore few ideas of application.

By utilising signed butterfly bipartite graphs in any network analysis(which fits in the boundaries of sense and meaning), we can investigate various aspects of network dynamics over which a signed butterfly bipartite graph may provide a suitable framework for capturing various relationships in networks.

In our graphs for all case studies, one set of nodes represents a group of an entity and the other set represents another group related to it. There are edges between nodes of different groups  with weight 1 is represented by positive edges, while weight 0 is represented by negative edges. The very definition of bipartite structure ensures that positive and negative edges only connect nodes from different groups, and not within the same group.


\subsection{Case Study $1$}
%Commented by Aman
% The case study 1 focuses on the analysis of signed butterflies in a bipartite graph of movie-actor network. By examining the presence and characteristics of signed butterflies, we aim to understand their significance in improving on the movie success probability, which in our case is derived from its IMDb rating.
%Edit by Aman
We conduct a case study for counting balanced butterflies in a singed bipartite graph of \textit{movie-actor} network. %Provide a citation for the dataset 
Counting the number of balanced butterflies is able to address many of the frequently asked interesting questions using such data set. \textbf{Q1}) Popularity/Influence of the actors. \textbf{Q2}) Collaboration between two actors. \textbf{Q3}) Actor's versatility.
%Commented by Aman
%Speaking about our analysis and data set, the analysis involves a bipartite network representation of actors and movies, obtained from a modified data set sourced from Kaggle. The data set primarily includes information about actors' names, movies, and IMDb ratings. For the purpose of constructing the network, a binary sign value of 1 was assigned to graph connections where the IMDb score for a movie was greater than or equal to 6, while a value of 0 was assigned otherwise. For the identification of each actor individually, we have given a unique id to each actor. We have used the proposed algorithm given in the paper, with few modification according to the utility, to count the number of balanced butterflies for each actor.

%Edit by Aman
The present some modifications to the original actor-movie data set so as to convert it in a proper signed bipartite network. The characteristics of the resulting data set used are as follows. It is composed of two distinct set of vertices, i.e., actors and movies (unique ID). Two vertices are connected by an edge if an actor as participated in a movie, and the binary edge weight $0$ or $1$ represent the positive or negative relation among the vertices. The binary sign value of $1$ is assigned to graph connections where the IMDb score for a movie was $\geq 6$, while a value of $0$ was assigned otherwise. We now study the three questions for our case study.
%Commented by Aman
%The applications of the algorithm can be used to do a data analysis on any relation that can be defined on the lines of the definition of signed butterfly. The application worked on by us are as follows.

%Commented by Aman
%In our case study, on the data set described before, we quantified the popularity/influence of the actors using the algorithm. This was done by counting the number of balanced butterflies for each individual actor within the network. The balanced butterfly mentioned here is only formed by the edges with sign/weight as 1. A detailed description of the butterfly is- Actor u has done two movies v and x, which had a rating of more than 6, similarly, actor w has done the same two movies v and x, thus one can get the edges accordingly. This means, there exists edges between u-v, w-v, u-x and w-x with assigned edge signs. The pattern so formed is our required balanced butterfly. This measure of popularity , i.e., an actor acting in various high rating movies indicated high level of recognition and success which incorporates all practical aspects of world (as the data set was totally generic).
To answer Q1, we count the number of balanced butterflies for each individual actor within the network. The balanced butterfly mentioned here is only formed by the edges with sign/weight as $1$. 
A detailed description of the butterfly is- Actor $u$ has done two movies $v$ and $x$, which had a rating of more than $6$, similarly, actor $w$ has done the same two movies $v$ and $x$, thus one can get the edges accordingly. This means, there exists edges between $u-v$, $w-v$, $u-x$ and $w-x$ with assigned edge signs. The pattern so formed is our required balanced butterfly. This measure of popularity , i.e., an actor acting in various high rating movies indicated high level of recognition and success which incorporates all practical aspects of world (as the data set was totally generic).

From the data set, actor with ID 2(Johnny Depp) is having highest number of balanced butterflies with multiple actors. This hints that his popularity/influence in all aspects is very high.
begin{figure}
\begin{figure}
\centering
%\subfigure[Evaluating Movies]{
\includegraphics[width=0.46\textwidth]{result-graphs/A.png}
%\vspace*{-3mm}
\caption{Movies by Actor 2(Johnny Depp)}
\label{fig:all}
%\vspace*{-2mm}
%\end{centering}
\end{figure}
Another application of the algorithm on the described data set is analysis on collaborative patterns between two actors. All sets of two distinct actors {u,w} were considered for this analysis and all the balanced butterflies (with all edges with sign 1) with the actors from a set were counted. The results of this analysis was used to get metric on potential collaborations for selection of actors of a movie, giving which collaboration was likely to be more successful over the others.
Actor 195 and 1024 are having highest number of balanced butterflies formed together which means this pair could give a higher chance of success for a new movie. The output set of pairs can be played with and a rigorous statistical analysis over the collaboration using the output can give deep insights over collaborative patterns.
\begin{figure}
\centering
%\subfigure[Evaluating Movies]{
\includegraphics[width=0.46\textwidth]{result-graphs/B.png}
%\vspace*{-3mm}
\caption{Movies by Actor 2(Johnny Depp)}
\label{fig:all}
%\vspace*{-2mm}
%\end{centering}
\end{figure}



A proposed application is analysis of actor versatility. An assessment on the diversity of balanced butterflies per actor for a specific genre can give us a potential versatility indicator. For example, an actor who has a high number of balanced butterflies in a non genre specific settings may have an expertise and success in several genres or styles. On the other hand, an actor with high number of balanced butterflies in a genre specific settings may have honed their skills in that particular field and are likely to be more successful. 

Another proposed application can be network centrality. The centrality of each actor inside the bipartite graph may be determined by analysing the balanced butterflies for each actor. Actors with a lot of balanced butterflies may be critical connections between various regions of the graph. A analysis on the count of balanced butterflies can be applied further on the concepts of network centrality to extend the existing metrics.


\label{label:expsetting}
\noindent
\begin{table*}[ht]
\small
\caption{\label{table:datasets}
Results of Actor Movie}
\vspace*{-4mm}
\begin{center}
%\scalebox{0.888}{
\resizebox{17cm}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
$Actor-Johnny Depp$  & $Jennifer Lawrence$ & $Actor-Jason Flemyng
$ & $Actor-Aidan Turner
$  \\
%& $\var_a$ & $\var_b$ & $\var_{min}$\\
%\hline
 $15(BBF)$ & $12(BBF)$ & $7(BBF)$ & $6(BBF)$ \\
\hline
$Pirates of the Caribbean: The Curse of the Black Pearl (8.1)$ & $X-Men: Days of Future Past(8)$ & $Lock, Stock and Two Smoking Barrels
(8.2)$ & $The Hobbit: The Desolation of Smaug(7.9)$ \\
\hline
$Platoon (8.1)$ & $Star Trek VI: The Undiscovered Country (7.2)$ & $The Curious Case of Benjamin Button (7.8)$ & $The Hobbit: An Unexpected Journey(7.9)$ \\
\hline
$Edward Scissorhands (7.9)$ & $Silver Linings Playbook(7.8)$ & $Rob Roy(6.9)$ & $The Hobbit: The Battle of the Five Armies(7.5)$ \\
\hline
$Ed Wood(7.9)$ & $X-Men: First Class(7.8)$ & $From Hell(6.8)$ & $The Mortal Instruments: City of Bones(6)$ \\
\hline
$Donnie Brasco(7.8)$ & $The Hunger Games: Catching Fire(7.6)$ & $Mean Machine(6.5)$ & $ $ \\
\hline
$Finding Neverland(7.8)$ & $X-Men: Apocalypse(7.3)$ & $Transporter 2(6.3)$ & $ $ \\
\hline
$What's Eating Gilbert Grape(7.8)$ & $The Hunger Games(7.3)$ & $Deep Rising
(6)$ & $ $ \\
\hline
$Fear and Loathing in Las Vegas(7.7)$ & $American Hustle(7.3)$ & $Clash of the Titans(5.8)$ & $ $ \\
\hline
$Blow(7.6)$ & $Winter's Bone(7.2)$ & $Ironclad(6.2)$ & $ $ \\
\hline
$A Nightmare on Elm Street(7.5)$ & $The Beaver(6.7)$ & $Mirrors(6.2)$ & $ $ \\
\hline

\end{tabular}}
\end{center}
%\vspace{-11}}
\end{table*}



\remove{
\label{label:expsetting}
\noindent
\begin{table*}[ht]
\small
\caption{\label{table:datasets}
Results of Actor Movie}
\vspace*{-4mm}
\begin{center}
%\scalebox{0.888}{
\resizebox{17cm}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
$Actor-Johnny Depp$  & $Actor-Nichelle Nichols
$ & $Actor-Jason Flemyng
$ & $Actor-Aidan Turner
$  \\
%& $\var_a$ & $\var_b$ & $\var_{min}$\\
%\hline
 $15(BBF)$ & $13(BBF)$ & $7(BBF)$ & $6(BBF)$ \\
\hline
$Pirates of the Caribbean: The Curse of the Black Pearl (8.1)$ & $Star Trek II: The Wrath of Khan(7.7)$ & $Lock, Stock and Two Smoking Barrels
(8.2)$ & $The Hobbit: The Desolation of Smaug(7.9)$ \\
\hline
$Platoon (8.1)$ & $Star Trek VI: The Undiscovered Country (7.2)$ & $The Curious Case of Benjamin Button (7.8)$ & $The Hobbit: An Unexpected Journey(7.9)$ \\
\hline
$Edward Scissorhands (7.9)$ & $Star Trek IV: The Voyage Home (7.3)$ & $Rob Roy(6.9)$ & $The Hobbit: The Battle of the Five Armies(7.5)$ \\
\hline
$Ed Wood(7.9)$ & $Star Trek III: The Search for SpockÂ(6.6)$ & $From Hell(6.8)$ & $The Mortal Instruments: City of Bones(6)$ \\
\hline
$Donnie Brasco(7.8)$ & $Star Trek: The Motion Picture(6.4)$ & $Mean Machine(6.5)$ & $ $ \\
\hline
$Finding Neverland(7.8)$ & $Star Trek V: The Final Frontier(5.4)$ & $Transporter 2(6.3)$ & $ $ \\
\hline
$What's Eating Gilbert Grape(7.8)$ & $Snow Dogs(5.1)$ & $Deep Rising
(6)$ & $ $ \\
\hline
$Fear and Loathing in Las Vegas(7.7)$ & $ $ & $Clash of the Titans(5.8)$ & $ $ \\
\hline
$Blow(7.6)$ & $ $ & $Ironclad(6.2)$ & $ $ \\
\hline
$A Nightmare on Elm Street(7.5)$ & $ $ & $Mirrors(6.2)$ & $ $ \\
\hline

\end{tabular}}
\end{center}
%\vspace{-11}}
\end{table*}

}

\noindent


\remove{
\subsection{Case Study 2}
This case study contains proposed analysis applications on user product data. The must be converted to a bipartite graph and the relations by and by will be drawn on the definition of a signed butterfly.

Through use of signed butterfly structure, a wide spectrum of analysis on the associations between users and products can facilitate the identification of prevalent and emergent products.The examination of the frequency and intensity of interactions  can give analysis of inclinations, purchasing behaviours, and the process of product adoption. The integration of these various analyses facilitates informed decision-making in areas such as inventory management, product development, marketing strategies, and comprehension of user behaviour within the framework of product popularity and trends.

Temporal changes and patterns in the relationships between users and products can be derived or analysed using signed butterfly counting. Comparison of the user-product data from the recent years and with the data from the previous year is proposed.

An already possibly in use application is product recommendation using user segmentation. The connections between users and products defined on the lines of signed butterfly can be put to collaborative filtering to suggests product which are popular among similar taste users.
This can further be expanded to community detection, where community detection algorithms form groups of users with like minded interests and preferences.

The above propositions are presented as potential avenues for investigating the butterfly framework within the realm of user-generated product data.
}

